Near-Optimal Detection in MIMO Systems using Gibbs Sampling

In this paper we study a Markov Chain Monte Carlo (MCMC) Gibbs sampler for solving the integer least-squares problem. In digital communication the problem is equivalent to performing Maximum Likelihood (ML) detection in Multiple-Input Multiple-Output (MIMO) systems. While the use of MCMC methods for such problems has already been proposed, our method is novel in that we optimize the "temperature" parameter so that in steady state, i.e. after the Markov chain has mixed, there is only polynomially (rather than exponentially) small probability of encountering the optimal solution. More precisely, we obtain the largest value of the temperature parameter for this to occur, since the higher the temperature, the faster the mixing. This is in contrast to simulated annealing techniques where, rather than being held fixed, the temperature parameter is tended to zero. Simulations suggest that the resulting Gibbs sampler provides a computationally efficient way of achieving approximative ML detection in MIMO systems having a huge number of transmit and receive dimensions. In fact, they further suggest that the Markov chain is rapidly mixing. Thus, it has been observed that even in cases were ML detection using, e.g. sphere decoding becomes infeasible, the Gibbs sampler can still offer a near-optimal solution using much less computations.

==> Conclusion/Conclusion.tex <==
\section{Conclusion}
\label{sec:Conclusion}
In this paper we considered solving the integer
least-squares problem using Monte Carlo Markov Chain Gibbs
sampling. The novelty of the proposed MCMC method is that, unlike simulated 
annealing techniques, we have a fixed temperature parameter in all the
iterations, with the property that after the Markov chain has mixed,
the probability of encountering the optimal solution is only
polynomial small (i.e. not exponentially small). We further compute
the optimal (here largest) value of the temperature parameter that
guarantees this. Simulation results indicate the
sensitivity of the method to the choice of the temperature parameter
and show that our computed value gives a very good approximation to
its optimal value. Investigating whether the Markov chain mixes in
polynomial time for this choice of temperature parameter is currently
under investigation.

==> Finding_optimal_alpha/Value_of_alpha.tex <==
\subsection{Value of $\alpha$}

Note that from (\ref{Eq:Jensen_part5}) it is clear that the larger
$\beta$ is, the larger $\pi_{-\oneb}$ is. Therefore, the range of
$\alpha$ that gives a polynomially small probability to $\pi_{-\oneb}$
is 
\begin{equation}
\frac{\alpha^2}{1-\frac{1}{\alpha^2}} \geq \frac{2\SNR}
{\ln N -\ln\ln N -\ln\zeta}. 
\end{equation}
It can be shown that in the regime, $\SNR>2\ln N$, the above quadratic
inequality in $\alpha$ has two positive real solutions, $\alpha_+\geq
\alpha_-$, and that the inequality holds for all
$\alpha\in[\alpha_-,\alpha_+]$. 

We know that, the larger $\alpha$ is, the faster the Markov chain
mixes.\footnote{In general, there is a trade-off between
faster mixing time of the Markov chain (due to an increase of
$\alpha$) versus slower encountering the optimal solution in
steady-state. In fact, at infinite temperature our algorithm reduces
to a random walk in a hypercube which mixes in $O(N\ln N)$ time.}
Therefore it is reasonable that we choose the largest 
permissible value for $\alpha$, i.e., $\alpha_+$. 

Figures \ref{fig:alpha_vs_SNR_N=10} and
\ref{fig:alpha_vs_SNR_N=50} show the values of $\alpha_+$
and $\alpha_-$ as a function of $\SNR$ for systems with $N=10$ and $N=50$, when we have $\zeta = 1/\ln N$. 
\begin{figure}[btp]
 \center
 \includegraphics[width=2.55in]{Figures/Value_of_alpha_vs_SNR_for_N=10_zeta=logN-1.eps}
 \vspace{-2mm}
\caption{Value of $\alpha$ vs.~$\SNR$ for system size $N=10$.}
\label{fig:alpha_vs_SNR_N=10}
\vspace{-2mm}
\end{figure}

\begin{figure}[htbp]
 \center
% \vspace{-35mm}
 \includegraphics[width=2.55in]{Figures/Value_of_alpha_vs_SNR_for_N=50_zeta=logN-1.eps}
 \vspace{-2mm}
\caption{Value of $\alpha$ vs.~$\SNR$ for system size $N=50$.}
\label{fig:alpha_vs_SNR_N=50}
\vspace{-2mm}
\end{figure}

\subsection{Mixing time of Markov Chain}
One open question is whether the Markov chain is rapidly mixing when 
using the strategy above for choosing $\alpha$. This
is something we are currently investigating, and the simulations
presented in Section \ref{sec:sim_results} seem to indicate that this
is the case. Furthermore, the
simulations also suggest that the computed value of $\alpha$ is very
close to the optimal choice, even in the case where the condition
$\SNR>2\ln(N)$ is not satisfied.  

==> Finding_optimal_alpha/finding_optimal_alpha.tex <==
\section{Computing the optimal $\alpha$}
\label{sec:comp_opt_alpha}

Assuming that the vector $\sb = -\oneb$ has been transmitted, the
probability of finding this solution {\em after the Markov chain has
  mixed} is simply $\pi_{-\oneb}$, the steady-state probability of
being in the all $-1$ state. Clearly, if this probability is
exponentially small, it will take exponentially long for the Gibbs
sampler to find it. We will therefore insist that the mean of
$\pi_{-\oneb}$ be only polynomially small. 

\input{Finding_optimal_alpha/mean_steady_state.tex}
\input{Finding_optimal_alpha/Value_of_alpha.tex}

==> Finding_optimal_alpha/mean_steady_state.tex <==
\subsection{Mean of $\pi_{-\oneb}$}

This calculation has a lot in common with the one
given in Section \ref{sec:P_error}. Note that the steady state value
of $\pi_{-\oneb}$ is simply 
%\begin{eqnarray}
\begin{subequations}
\label{Eq:mean_of_pi}
\begin{align}
\pi_{-\oneb} & = \frac{e^{-\frac{1}{2\alpha^2}\left\|\yb+\sqrt{\frac{\SNR}{N}}\Hb \oneb\right\|^2}}
{\sum_\sb e^{-\frac{1}{2\alpha^2}\left\|\yb+\sqrt{\frac{\SNR}{N}}\Hb \sb\right\|^2}} \\
& = \frac{e^{-\frac{1}{2\alpha^2}\left\|\upsib\right\|^2}}
{\sum_\sb e^{-\frac{1}{2\alpha^2}\left\|\upsib+\sqrt{\frac{\SNR}{N}}\Hb(\sb-\oneb)\right\|^2}} \\
& = \frac{e^{-\frac{1}{2\alpha^2}\left\|\upsib\right\|^2}}
{\sum_{\delb} e^{-\frac{1}{2\alpha^2}\left\|\upsib+2\sqrt{\frac{\SNR}{N}}\Hb \delb\right\|^2}} \\
& = \frac{1} {\sum_{\delb} e^{-\frac{1}{2\alpha^2}\left(
\left\|\upsib+2\sqrt{\frac{\SNR}{N}}\Hb\delb\right\|^2-\|\upsib\|^2\right)}} \ ,
\end{align}
\end{subequations}
%\end{eqnarray}
where $\delb$ is a vector of zeros and ones and the summations (over
$\sb$ and $\delb$) are over $2^n$ terms.

Now, by Jensen's inequality
\begin{subequations}
\label{Eq:Expetaion_of_pi}
\begin{align}
E \left\{ \pi_{-\oneb} \right\} & \geq \frac{1}{E \left\{ \frac{1}{\pi_{-\oneb}}\right\} } \\
 & =  
\frac{1}{E \left\{ \sum_{\delb} e^{-\frac{1}{2\alpha^2}\left(
\left\|\upsib+2\sqrt{\frac{\SNR}{N}}\Hb \delb\right\|^2-\left\|\upsib\right\|^2\right)} \right\}} \\
& = \frac{1}
{\sum_{\delb} E \left\{ e^{-\frac{1}{2\alpha^2}\left(
\left\|\upsib+2\sqrt{\frac{\SNR}{N}}\Hb \delb\right\|^2-\left\|\upsib\right\|^2\right) }\right\} } \\
& = \frac{1}{1+\sum_{\delb \neq 0}
\left(\frac{1}{1+4\frac{\SNR\left\|\delb\right\|^2}{N}
\frac{1}{\alpha^2}(1-\frac{1}{\alpha^2})}\right)^{N/2}} \label{Eq:Jensen_part4} \\
& = \frac{1}{1+\sum_{i=1}^N\left(\begin{array}{c} N \\ i \end{array} \right)
\left(\frac{1}{1+\frac{\beta i}{N}}\right)^{N/2}} \label{Eq:Jensen_part5} \ .
\end{align}
\end{subequations}
In \eqref{Eq:Jensen_part4} we have used Lemma \ref{lem:g-i} and in
 \eqref{Eq:Jensen_part5} we have defined $\beta \triangleq
 4\SNR\frac{1}{\alpha^2}(1-\frac{1}{\alpha^2})$. 
 While it is possible to focus on the linear and sublinear terms in the
above summation separately, to give conditions for $E \left\{
 \pi_{-\oneb} \right\}$ to have 
the form of $1/\mbox{poly}(N)$, we will be interested in the exact
exponent and so will need a more accurate estimate. To do
this we shall use saddle point integration. Note that
\begin{equation*}
\left(\begin{array}{c} N \\ i \end{array} \right)
\left(\frac{1}{1+\frac{\beta i}{N}}\right)^{N/2} \\ 
\approx e^{N H(\frac{i}{N})-\frac{N}{2}\ln\left(1+\frac{\beta i}{N}\right)} \ ,
\end{equation*}
where again $H(\cdot)$ represents the entropy in ``nats''. And so the
summation in the denominator of \eqref{Eq:Jensen_part5} can be 
approximated as a Stieltjes integral:
\begin{subequations}
\begin{align}
\sum_{i=1}^N\left(\begin{array}{c} N \\ i \end{array} \right)
\left(\frac{1}{1+\frac{\beta i}{N}}\right)^{N/2} & \approx
N\sum_{i=1}^Ne^{N H(\frac{i}{N})-\frac{N}{2}\ln\left(1+\frac{\beta
i}{N}\right)}\frac{1}{N} \\ 
& \approx N\int_0^1e^{N H(x)-\frac{N}{2}\ln\left(1+\beta x\right)}dx \ .
\end{align}
\end{subequations}
For large $N$, this is a saddle point integral and can be approximated
by the formula
\be
\int_0^1e^{N f(x)}dx \approx \sqrt{\frac{2\pi}{N|f''(x_0)|}}e^{N f(x_0)} \ , 
\label{Eq:saddlepoint}
\ee
where $x_0$, is the saddle point of $f(\cdot)$, i.e.,$f'(x_0) = 0.$
In our case,
\[ f(x) = -x\ln x-(1-x)\ln(1-x)-\frac{1}{2}\ln(1+\beta x) \ , \]
and so
\[ f'(x) = \ln\frac{1-x}{x}-\frac{1}{2}\frac{\beta}{1+\beta x} \ . \]
In general, it is not possible to solve for $f'(x_0) = 0$ in closed
form. However, in our case, if we assume that $\beta = 4\SNR
\frac{1}{\alpha^2}(1-\frac{1}{\alpha^2})\gg 1$ (which is true
since the SNR grows at least logarithmically),
then it is not too hard to verify that the saddle point is given by
\be
x_0 = e^{-\frac{\beta}{2}} \ .
\ee
And hence $f(x_0) = $
\begin{equation*}
\begin{split}
& -e^{-\frac{\beta}{2}}\ln e^{-\frac{\beta}{2}}
-(1-e^{-\frac{\beta}{2}})\ln(1-e^{-\frac{\beta}{2}}) 
- \frac{1}{2}\ln(1+\beta e^{-\frac{\beta}{2}}) \\
& \approx
\frac{\beta}{2}e^{-\frac{\beta}{2}}+e^{-\frac{\beta}{2}}-\frac{1}{2}
\beta e^{-\frac{\beta}{2}} 
= e^{-\frac{\beta}{2}} \ ,
\end{split}
\end{equation*}
and further plugging $x_0$ into $f''(x) = -\frac{1}{x}
-\frac{1}{1-x}-\frac{1}{2}\frac{\beta^2}{(1+\beta x)^2}$, yields
\be
f''(x_0) \approx -e^{\frac{\beta}{2}}-1+\frac{1}{2}\beta^2 \approx
-e^{\frac{\beta}{2}} \ . 
\ee
Replacing these into the saddle point expression in \eqref{Eq:saddlepoint} show that
\begin{equation}
\label{Eq:sum_approx_by_saddl}
\sum_{i=1}^N \left(\begin{array}{c} N \\ i \end{array} \right)
\left(\frac{1}{1+\frac{\beta i}{N}}\right)^{N/2} \approx 
\sqrt{2\pi/N} \exp{\left(N e^{-\frac{\beta}{2}}-\frac{\beta}{4}\right)} \ . 
\end{equation}
We want $E \left\{ \pi_{-\oneb} \right\}$ to behave as $\frac{1}{N^\zeta}$ and according to \eqref{Eq:Expetaion_of_pi} this means
that we want the expression in \eqref{Eq:sum_approx_by_saddl} to behave as $N^{\zeta}$. Let us take
\[ e^{Ne^{-\frac{\beta}{2}}} = N^{\zeta} \ . \]
Solving for $\beta$ yields
\be 
\beta = 4\SNR \frac{1}{\alpha^2}\left(1-\frac{1}{\alpha^2}\right) =
2\left(\ln N -\ln\ln N -\ln\zeta \right) . 
\ee
Incidentally, this choice of $\beta$ yields $e^{-\frac{\beta}{4}}
\approx \frac{1}{\sqrt{N}}$, 
and so we have the following result.

\begin{lemma}[Mean of $\pi_{-\oneb}$] If $\alpha$ is chosen such that 
\be
\label{EQ:Alpha_expression}
\frac{\alpha^2}{1-\frac{1}{\alpha^2}} = \frac{2\SNR}
{\ln N -\ln\ln N -\ln\zeta} \ ,
\ee
then
\be
\label{Eq:Mean_pi_lemma}
E \left\{\pi_{-\oneb} \right\} \geq N^{-\zeta} \ .
\ee
\end{lemma}

==> Gibbs_sampling/Gibbs_sampling.tex <==
\section{Gibbs Sampling}
\label{sec:Gibbs_sampling}
One way of solving the optimization problem given in
\eqref{EQ:Original_minimization_problem} is by using Markov Chain
Monte Carlo (MCMC) simulations, which asymptotically converge to the
optimal solution \cite{Mackay_03}. More specifically, the MCMC
detector we investigate 
here is the Gibbs sampler, which computes the conditional probability
of each symbol in the constellation set at the $j$th index in the
estimated symbol vector. This conditional probability is obtained by
keeping the $j-1$ other values in the estimated symbol vector
fixed. Thus, in $k$th iteration the probability of the $j$th symbol
adopts the value $\omega$, is given as 
\begin{equation}
\label{Eq:Prob_of_symbol_MCMC}
% p\left( {\hat{\sb}_j^{(k)} = \omega \left|{ \hat{\sb}^{(k-1)}, \yb,
% \Hb}\right.} \right) = 
p\left( {\hat{\sb}_j^{(k)} = \omega \left|{ \theta }\right.} \right) =
\frac{e^{-\frac{1}{2\alpha^2} \left\| \yb - \sqrt{\frac{\SNR}{N}} \Hb
    \tilde{\sb}_{j \left|{\omega}\right.} \right\|^2   }}{
  \sum\limits_{\tilde{\sb}_{j \left|{\tilde{\omega}}\right.} \in
    \Omega}{e^{-\frac{1}{2\alpha^2} \left\| \yb -
      \sqrt{\frac{\SNR}{N}} \Hb \tilde{\sb}_{j \left|{ \tilde{\omega}
	}\right.} \right\|^2 } }}  \ , 
\end{equation}
where $\tilde{\sb}_{j \left|{\omega}\right. }^T \triangleq
\left[\hat{\sb}_{1:j-1}^{(k)}, \omega, \hat{\sb}_{j+1:N_T}^{(k-1)}
  \right]^T$ and where we for simplicity have introduced $\theta =
\left\{ \hat{\sb}^{(k-1)}, \yb, \Hb \right\}$.\footnote{When we
  compute the probability of symbol $\omega$ at the $j$'th position,
  we more precisely condition on the symbols $\hat{\sb}_{1:j-1}^{(k)}$
  and $\hat{\sb}_{j+1:N_T}^{(k-1)}$, but to keep the notation simple,
  we do not explicitly state that in the equations above.} $\alpha$
represents a tunable positive parameter which controls the mixing time
of the Markov chain, this parameter is also sometimes called the
"temperature". The  larger $\alpha$ is the faster the mixing time of
the Markov chain will be, but as we will show in the paper, there is
an upper limit on $\alpha$, in order to ensure that the probability of
finding the optimal solution in steady state is not exponentially
small. The MCMC method will with probability $p\left(
{\hat{\sb}_j^{(k)} = \omega \left|{\theta}\right.} \right)$ keep
$\omega$ at the $j$'th index in estimated symbol vector, and compute
conditional probability the $(j+1)$th index in a similar fashion. We
define one iteration of the Gibbs sampler as a randomly-ordered update of
all the $j = \left\{1, \ldots, N_T \right\}$ indices in the estimated
symbol vector $\hat{\sb}$.\footnote{We need a randomly-ordered update
  for the Markov chain to be reversible and for our subsequent
  analysis to go through. It is also possible to just randomly select
  a symbol $j$ to update, without insisting that a full sequence be
  done. This also makes the Markov chain reversible and has the same
  steady state distribution. In practice a fixed, say sequential,
  order can be employed, although the Markov chain is no longer
  reversible. Note that our theoretical analysis is assuming randomly selected  
symbol updates for analytical convenience. In our experimental  
section we used a sequential updating order which empirically yields a slight  
convergence acceleration.} The initialization of the symbol vector 
$\hat{\sb}^{(0)}$ can either be chosen randomly or, alternatively,
e.g. the zero-forcing solution can be used.

%%%%%%%%%%%%%%%%%%%%%%%%%%%% New subsection %%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Complexity of the Gibbs sampler}
\label{subsec:Gibbs_complexity}
The conditional probability for the $j$'th symbol in \eqref{Eq:Prob_of_symbol_MCMC} can be computed efficiently by reusing the result obtained for the $j-1$'th symbol, when we evaluate $\left\| \yb - \sqrt{\SNR/N} \Hb \tilde{\sb}_{j \left|{\omega}\right.} \right\|^2$. Since we are only changing the $j$'th symbol in the symbol vector, the difference $\db_{j} \triangleq \yb - \sqrt{\SNR/N} \Hb \tilde{\sb}_{j \left|{\omega }\right.} $ can be expressed as
\begin{equation}
\label{EQ:difference_for_norm}
 \db_j = \db_{j-1} - \sqrt{\frac{\SNR}{N}} \Hb_{1:N,j} \Delta s_{j\left|{\omega}\right.} \ ,
\end{equation}
where $\Delta s_{j\left|{\omega}\right.} \triangleq s_{j \left|{\omega}\right.}^{(k)} - s_{j \left|{ \tilde{\omega} }\right.}^{(k-1)}$.  Thus, the computation of conditional probability of certain symbol in the $j$'th position costs $2N$ operations, where we define an operation as a Multiply and Accumulate (MAC) instruction.\footnote{We need to compute both the inner product $\db_j^T \db_j$ and the product $\Hb_{1:N,j} \Delta s_{j\left|{\omega}\right.}$.} This leads to a complexity of $\bigO \left( 2N^2[\left|\Omega \right| -1 ]\right)$ operations per iteration. For further details on the implementation of the Gibbs sampler see \cite{Laraway_Farhang-Boroujeny_IEEE_09}.



==> Introduction/Introduction.tex <==
\section{Introduction}
\label{sec:Introduction}
The problem of performing Maximum Likelihood (ML) decoding in digital
communication has gained much attention over the years. One method to
obtain the ML solution is Sphere Decoding (SD)
\cite{Hochwald_Ten-Brink_03, Hassibi_1, Hassibi_2,Agrell_et_al_02,
  Damen_et_al}. Over a wide range of Signal-to-Noise Ratios ($\SNR$)s
the average complexity of SD is significantly smaller than exhaustive
search detectors, but in worst case the complexity is still
exponential \cite{Ottersten_05}. Thus, in scenarios with poor $\SNR$
or in Multiple-Input Multiple-Output (MIMO) systems with huge transmit
and receive dimensions, even SD can be infeasible. A way to overcome
this problem is to use approximate Markov Chain Monte Carlo (MCMC)
detectors instead, which asymptotically can provide the optimal
solution, \cite{Robert_MC_Stat_methods_04, Haggstrom_02}. Gibbs
sampling (also known as Glauber dynamics) is one MCMC method, which is
used for sampling from distributions of multiple dimensions. The Gibbs
sampler has among others been proposed for detection purposes in wireless
communication in \cite{Zhu_Farhang_Boroujeny_05, Farhang_Boroujeny_06, Wang_Poor_03, Chen_Wang_2002} (see also the references therein). The scope of this
paper is to describe and analyse a new way of solving the integer
least-squares problem using MCMC. It will be shown that the method can
be used for achieving a near-optimal and computationally efficient
solution of the problem, even for systems having a huge dimension. 

The paper is organized as follows; In Section \ref{sec:System_model}
we present the system model that will be used throughout the
paper. The MCMC method is described in Section
\ref{sec:Gibbs_sampling} and in Section \ref{sec:P_error} we analyse
the probability of error for the ML detector. Section
\ref{sec:comp_opt_alpha} treats the optimal selection of the
temperature parameter $\alpha$, while the simulation results are given
in Section \ref{sec:sim_results} and some concluding remarks are found
in Section \ref{sec:Conclusion}. 

==> Prob_of_err_ML/Prob_of_err_ML.tex <==
\section{Probability of Error}
\label{sec:P_error}

In this paper, we are interested in evaluating the performance of the
aforementioned Gibbs sampler, compared to the ML solution. To ease our
analysis, we will assume that the ML detector finds the correct
transmitted vector. Before we derive the probability of error for the
ML detector, we will state a lemma which we will make repeated use of. 
\begin{lemma}[Gaussian Integral] \label{Lem:Gaussian_integral} Let $\vb$ and $\xb$ be independent
  Gaussian random vectors with distribution ${\cal N}(\zerob,\Ib_N)$
  each. Then, if $1-2a^2\eta(1+2\eta)>0$,
\be
E \left\{ e^{\eta\left(\|\vb+a\xb\|^2-\|\vb\|^2\right)} \right\}=
  \left(\frac{1}{1-2a^2\eta(1+2\eta)}\right)^{N/2}. 
\ee
\label{lem:g-i}
\end{lemma}
\begin{proof}
\label{Pro:Gaussian_integral}
See Appendix \ref{subsec:Gaussian_integral} for a detailed proof.
\end{proof}
\vspace{2mm}
Assuming that the vector $\sb= -\oneb$ was transmitted, the ML
detector will make an error if there exists a vector $\sb\neq -\oneb$
such that 
\[
\left\|\yb-\sqrt{\frac{\SNR}{N}}\Hb\sb\right\|^2\leq 
\left\|\yb+\sqrt{\frac{\SNR}{N}} \Hb\oneb\right\|^2 = \|\upsib\|^2 \ .
\] In other words,
\begin{eqnarray*}
P_e & = & \mbox{Prob}\left(\left\|\yb-\sqrt{\frac{\SNR}{N}}\Hb\sb\right\|^2\leq
  \|\upsib\|^2 \right) \\%% \mbox{for some $\sb\neq -\oneb$}\right)  \\ 
& = & \mbox{Prob}\left(\left\|\upsib+\sqrt{\frac{\SNR}{N}}\Hb(-\oneb-\sb)\right\|^2\leq 
  \|\upsib\|^2 \right) \ ,\\%% \mbox{for some $\sb\neq -\oneb$}\right) \\
\end{eqnarray*}
for some $\sb\neq -\oneb$, which can be formulated as
\begin{eqnarray*}
P_e & = &  \mbox{Prob}\left(\left\|\upsib+2\sqrt{\frac{\SNR}{N}}\Hb\delb\right\|^2\leq 
  \|\upsib\|^2 \right) \ ,%% \mbox{for some $\delb\neq 0$}\right).
\end{eqnarray*}
for some $\delb\neq 0$. Note that in the above equation $\delb$ is a vector of zeros and
$-1$'s. Now using the union bound
\be
P_e \leq \sum_{\delb\neq 0}
\mbox{Prob}\left(\left\|\upsib+2\sqrt{\frac{\SNR}{N}}\Hb\delb\right\|^2\leq 
  \|\upsib\|^2\right). 
\ee
We will use the Chernoff bound to bound the quantity inside the
summation. Thus,
\begin{subequations}
\begin{align}
& \mbox{Prob}\left(\left\|\upsib+2\sqrt{\frac{\SNR}{N}}\Hb\delb\right\|^2 \leq \|\upsib\|^2\right) \\ 
& \leq E \left\{ e^{-\beta  \left(\left\|\upsib+2\sqrt{\frac{\SNR}{N}}\Hb\delb\right\|^2-\|\upsib\|^2\right)} \right\} \\ 
& = \left(\frac{1}{1+8\frac{\SNR\|\delb\|^2}{N} \beta(1-2\beta)}\right)^{N/2},
\end{align}
\end{subequations}
where $\beta\geq 0$ is the Chernoff parameter, and where we have used
Lemma \ref{lem:g-i} with $\eta = -\beta$ and 
$a = 2\sqrt{\frac{\SNR\|\delb\|^2}{N}}$, since 
\[ E \left\{ \left(2\sqrt{\frac{\SNR}{N}}\Hb\delb\right)
\left(2\sqrt{\frac{\SNR}{N}}\Hb\delb\right)^* \right\} =
4\frac{\SNR\|\delb\|^2}{N} \Ib_N. \]
The optimal value for $\beta$ is $\frac{1}{4}$, which yields the
tightest bound
\be
\mbox{Prob}\left(\left\|\upsib+2\sqrt{\frac{\SNR}{N}}\Hb\delb\right\|^2\leq 
  \|\upsib\|^2\right) \leq \left(\frac{1}{1+\frac{\SNR\|\delb\|^2}{N}}
\right)^{N/2}.
\ee
Note that this depends only on $\|\delb\|^2$, the number of nonzero
entries in $\delb$. Plugging this into the union bound yields
\be
P_e \leq \sum_{i=1}^N \left( \begin{array}{c} N \\ i \end{array}
\right) \left(\frac{1}{1+\frac{\SNR i}{N}}
\right)^{N/2}.
\ee

Let us first look at the linear (i.e., $i$ proportional to $N$) terms
in the above sum. Thus,
\[ \left( \begin{array}{c} N \\ i \end{array}
\right) \left(\frac{1}{1+\frac{\SNR i}{N}}
\right)^{N/2} \approx
e^{N H(\frac{i}{N})-\frac{N}{2}\ln\left(1+\frac{\SNR i}{N}\right)}, \]
where $H(\cdot)$ is entropy in ``nats''. Clearly, if
$\lim_{N\rightarrow\infty}\SNR = \infty$, then the linear terms go to
zero (superexponentially fast). 

Let us now look at the sublinear terms. In particular, let is look at
$i=1$: 
\[ N\left(\frac{1}{1+\frac{\SNR}{N}}\right)^{N/2} \approx
N e^{-\SNR/2}. \]
Clearly, to have this term go to zero, we require that $\SNR>
2\ln N$. A similar argument shows that all other sublinear terms also go to
zero, and so.\footnote{Due to space constraints we only present a sketch of this bound. A
rigorous proof can be given using the saddle point method, similarly
to the proof in the next section.}

\begin{lemma}[SNR scaling] If $\SNR>2\ln N$, then
  $P_e\rightarrow 0$ as $N\rightarrow\infty$. 
\end{lemma}


==> Simulations/Simulations.tex <==
\section{Simulation Results}
\label{sec:sim_results}
%%%%%%%%Next figure %%%%%%%%%%%%%
\begin{figure}[tp]
	\centering
	\includegraphics[width=2.6in]{Figures/sim_MCMC_BER_vs_iter_Alphabet=ChType=RFS_N=10_SNRdB=10_MinErr=500.eps}
%\includegraphics[width=0.4\textwidth]{}
	\vspace{-2mm}
	\caption{BER vs. iterations, $10 \times 10$. $\SNR$ = 10 dB.}
	\label{fig:Sim_alpha_SNR=10}
	\vspace{-2mm}
\end{figure}
%%%%%%%%Next figure %%%%%%%%%%%%%
\begin{figure}[tp]
	\centering
  \includegraphics[width=2.6in]{Figures/sim_MCMC_BER_vs_iter_Alphabet=ChType=RFS_N=10_SNRdB=14_MinErr=500.eps}
	\vspace{-2mm}
	\caption{BER vs. iterations, $10 \times 10$ system. $\SNR$ = 14 dB.}
	\label{fig:Sim_alpha_SNR=14}
	\vspace{-2mm}
\end{figure}
In this section we present simulation results for a MIMO $N \times N$
system with a full square channel matrix containing i.i.d.~Gaussian
entries. In Fig. \ref{fig:Sim_alpha_SNR=10} and Fig.
\ref{fig:Sim_alpha_SNR=14} the Bit Error Rate (BER) of the Gibbs
sampler, initialized with a random $\sb$, has been evaluated as a
function of the number of iterations 
in a $10 \times 10$ system using a variety of $\alpha$ values. Thereby,
we can inspect how the parameter $\alpha$ affects the convergence rate
of the Gibbs sampler. 
The performance of the Maximum Likelihood (ML), the Zero-Forcing (ZF),
and the Linear Minimum Mean Square Error (LMMSE) detector has also
been plotted, to ease the comparison of the Gibbs sampler with
these. It is seen that the Gibbs sampler outperforms both the ZF and
the LMMSE detector after only a few iterations in all the presented
simulations, when the tuning parameter $\alpha$ is chosen
properly. Furthermore, it is observed that the parameter $\alpha$ has
a huge influence on the convergence rate and that the Gibbs sampler
converges toward the ML solution as a function of the
iterations.\footnote{It should be noted that the way we decode the
  symbol vector to a given iteration, is to select the symbol vector
  which has the lowest cost function in all the iterations up to that
  point in time.} The optimal value of $\alpha$ (in terms of
convergence rate) is quite close to the theoretical values from Fig. \ref{fig:alpha_vs_SNR_N=10} of $\alpha_+ =
2.7$ and $\alpha_+ = 4.6$ at $\SNR$'s at $10$ and $14 dB$, respectively. It is also observed that the performance of the Gibbs sampler is significantly deteriorated if the temperature parameter is chosen based on the $\SNR$ (and thereby on the noise variance), such that $\alpha = \sigma \triangleq 1/\SNR$. Thus, the latter strategy is clearly not a wise choice.\\
Figure \ref{fig:Sim_alpha_BER_vs_SNR_iter=100} shows the BER
performance for the MCMC detector for fixed number of iterations, $k =
100$. From the figure we see that the $\SNR$ has a significant
influence on the optimal choice of $\alpha$ given a fixed number of
iterations. 
%%%%%%%%Next figure %%%%%%%%%%%%%
\begin{figure}[tp]
	\centering
\includegraphics[width=2.6in]{Figures/sim_MCMC_BER_vs_SNR_Alphabet=ChType=RFS_N=10_iter=100_MinErr=500_BER.eps} 
\vspace{-2mm}
	\caption{BER vs. $\SNR$, $10 \times 10$. Number of iterations, $k = 100$.}
	\label{fig:Sim_alpha_BER_vs_SNR_iter=100}
	\vspace{-2mm}
\end{figure}
%-----------------
\\The performance of the Gibbs sampler is also shown for a
$50 \times 50$ system, which represents a ML decoding problem of huge
complexity where an exhaustive search would require $2^{50}
\approx 10^{15}$ evaluations. For this problem even the sphere decoder
has an enormous complexity under moderate $\SNR$.\footnote{In fact, it
  can be shown that, for $\SNR = \bigO(\ln N)$, the lower bound on the
  complexity of the sphere decoder obtained in \cite{Ottersten_05}
  is exponential.} Therefore, it has not been
possible to simulate the performance of this decoder within a
reasonable time and we have therefore ``cheated'' a little by
initializing the radius of the sphere to the minimum of either the
norm of the transmitted symbol vector or the solution found by the
Gibbs sampler. This has been done in order to evaluate the BER
performance of the optimal detector. Figure
\ref{fig:Sim_alpha_N=50_SNR=12} shows the BER curve as a function of
the iteration number, while Figure
\ref{fig:Sim_alpha_BER_vs_SNR_N=50_iter=500} illustrates the BER curve
vs. the $\SNR$. From Figure \ref{fig:Sim_alpha_N=50_SNR=12} we see
that there is a quite good correspondence between the simulated
$\alpha$ and the theoretical value $\alpha_+ = 2.6$ obtained from
Figure \ref{fig:alpha_vs_SNR_N=50}. 
%%%%%%%%Next figure %%%%%%%%%%%%%
\begin{figure}[tp]
	\centering
  \includegraphics[width=2.6in]{Figures/sim_MCMC_BER_vs_iter_Alphabet=ChType=RFS_N=50_SNRdB=12_MinErr=500.eps}
	\vspace{-2mm}
	\caption{BER vs. iterations, $50 \times 50$ system. $\SNR$ = 12 dB.}
	\label{fig:Sim_alpha_N=50_SNR=12}
	\vspace{-2mm}
\end{figure}
%%%%%%%%Next figure %%%%%%%%%%%%%
\begin{figure}[tb]
	\centering
\includegraphics[width=2.6in]{Figures/sim_MCMC_BER_vs_SNR_Alphabet=ChType=RFS_N=50_iter=500_MinErr=500_BER.eps} 
\vspace{-2mm}
	\caption{BER vs. \SNR, $50 \times 50$ system. Num. of iter., $k = 500$.}
	\label{fig:Sim_alpha_BER_vs_SNR_N=50_iter=500}
	\vspace{-2mm}
\end{figure}
\input{Simulations/Table_of_complexity.tex}
The average complexity (MAC pr. symbol vector) of the Gibbs sampler having a BER performance comparable with the ML detector is shown in Table \ref{Tab:Complexity_SD_vs_GS}. The SD has been included as a reference.\footnote{It has not been possible to simulate the SD for a $50\times50$ system when $SNR\leq10dB$ and, therefore, the complexity of $SNR=12 dB$ has been used a lower bound.} It is observed that the complexity of the Gibbs sampler is not affected by the $\SNR$ as much as the SD.

==> Simulations/Table_of_complexity.tex <==
\begin{table}[!tbp]  %Table template.
    %\vspace{-2mm}
    \centering
    \caption{Complexity of SD and Gibbs Sampler (GS).}
    \begin{tabular}[!h]{l| c| r r r}
        \hline \hline
                $N$ 		& Method  & $\SNR$ \hspace{3mm} 6 dB	& 10 dB	& 14 dB \\ 
                \hline
                %\vspace{1mm}               
         				\multirow{2}{*}{10} & GS 	& $9.8\cdot10^3$		& $10.9\cdot10^3$		&  $16.4\cdot10^3$ \\
         														& SD  & $10.0\cdot10^3$   & $1.7\cdot10^3$  	&  $1.5\cdot10^3$  \\
         				\hline
         				\multirow{2}{*}{50}	& GS 	& $7.6\cdot10^5$		& $9.5\cdot10^5$ 	 	&  $10.6\cdot10^5$   \\
         														& SD  & $\gg 1.9\cdot10^9$ & $\gg 1.9\cdot10^9$ &  $37.7\cdot10^5$   \\
                %\vspace*{1mm}
        \hline
     \end{tabular}
     \label{Tab:Complexity_SD_vs_GS}
     \vspace{-5mm}
\end{table}


==> Simulations/Table_of_opt_alpha.tex <==
\begin{table}[!tb]  %Table template.
    \centering
    \caption{Theoretical values of $\alpha$ for $N\rightarrow\infty$.}
    \begin{tabular}[!h]{l c c}
        \hline \hline
                \SNR & 10 dB & 14 dB \\ 
                \hline
                %\vspace{1mm}               
         				$\alpha_{+}$	& 2.7  &  4.6 \\
                %\vspace*{1mm}
        \hline
     \end{tabular}
     \label{tab:Selection_alpha}
\end{table}


==> System_model/System_model.tex <==
\section{System Model}
\label{sec:System_model}
We consider a real-valued block-fading MIMO antenna system, with $N$
transmit and $N$ receive dimensions, with know channel
coefficients.\footnote{For simplicity we have assumed that the receive and the transmit dimensions are the same, but the results presented in the paper can be generalized to cover different dimensions.} The received signal $\yb \in \Rbb^N$ can be expressed
as 
\begin{equation}
\label{EQ:sig_model_matrix} 
\yb = \sqrt{\frac{\SNR}{N}}{\Hb\sb} + \upsib \ ,
\end{equation}
where $\sb \in \Omega^{N}$ is the transmitted signal, and $\Omega$
denotes the constellation set. To simplify the derivations in the
paper we will assume that $\Omega = \left\{\pm 1\right\}$. $\upsib \in
\Rbb^{N}$ is the noise vector where each entry is Gaussian $\Nc
\left(0,1\right)$ and independent identically distributed (i.i.d.),
and $\Hb \in \Rbb^{N \times N}$ denotes the channel matrix with
i.i.d. $\Nc \left(0,1\right)$ entries. The normalization in
(\ref{EQ:sig_model_matrix}) guarantees that $\SNR$ represents the 
signal-to-noise ratio per receive dimension (which we define as the ratio of the total transmit energy per channel use divided by the per-component noise variance as described in among others \cite{Damen_et_al}). As explained further below, for analysis
purposes we will focus on the regime where 
$\SNR > 2\ln(N)$, in order to get the probability of error of the ML
detector to go to zero. Further, in our analysis, without loss of
generality, we will assume that the all minus one vector was
transmitted, $\sb = -\oneb$. Therefore 
\begin{equation}
\yb = \upsib-\sqrt{\frac{\SNR}{N}}\Hb\oneb \ .
\end{equation}

%\subsection{Optimization problem}
We are considering a minimization of the average error probability
$P\left({\bf e} \right) \triangleq P\left(\hat{\sb} \neq \sb \right)$,
which is obtained by performing Maximum Likelihood Sequence Detection
(here simply referred to as ML detection) given by 
\begin{equation}
\label{EQ:Original_minimization_problem}
 \hat{\sb} = \arg	\mathop {\text{min} }\limits_{\sb \in \Omega^{N}} \ \  \left\| \yb - \sqrt{\frac{\SNR}{N}}\Hb \sb \right\|^2 \ .
\end{equation}

